The impact of overbooking on a pre-trial risk assessment tool

Pre-trial risk assessment tools are used to make recommendations to judges about appropriate conditions of pre-trial supervision for people who have been arrested. Increasingly, there is concern about whether these models are operating fairly, including concerns about whether the models' input factors are fair measures of one's criminal activity. In this paper, we assess the impact of booking charges that do not result in a conviction on a popular risk assessment tool, the Arnold Public Safety Assessment. Using data from a pilot run of the tool in San Francisco, CA, we find that booking charges that do not result in a conviction (i.e. charges that are dropped or end in an acquittal) increased the recommended level of pre-trial supervision in around 27% of cases evaluated by the tool

==> all-comparison-prop.tex <==
% latex table generated in R 3.5.1 by xtable 1.8-4 package
% Wed Dec  4 11:33:45 2019
\begin{table}[ht]
\centering
\begin{tabular}{lrrrr}
  \hline
Subset & exclusions & bump-ups & nvca & rec \\ 
  \hline
All Cases & 20.9 & 17.0 & 10.9 & 27.4 \\ 
  Conv Dispo & 21.6 & 14.0 & 10.5 & 23.9 \\ 
   \hline
\end{tabular}
\caption{Percent of cases with a charge-based exclusion, charge-based bump-up, or higher recommendations due to unsubstantiated booking charges.} 
\label{tab:all-comparison-prop}
\end{table}


==> all-comparison-race.tex <==
% latex table generated in R 3.5.1 by xtable 1.8-4 package
% Wed Dec  4 11:33:45 2019
\begin{table}[ht]
\centering
\begin{tabular}{lllllll}
 Subset & Charges & group & exclusions & bump-ups & nvca & rec \\ 
  \hline
All Cases & Conviction & non-black & 7.9 & 8.2 & 7.7 & 2.4 \\ 
  All Cases & Conviction & black & 9.7 & 10.3 & 11.5 & 2.6 \\ 
   \hline
All Cases & Booking & non-black & 25.9 & 23.2 & 15.9 & 2.9 \\ 
  All Cases & Booking & black & 33.9 & 24.3 & 25.7 & 3.1 \\ 
   \hline
All Cases & Difference & non-black & 18 * & 15 * & 8.2 * & 0.5 * \\ 
  All Cases & Difference & black & 24.2 * & 14.1 * & 14.2 * & 0.5 * \\ 
   \hline
\hline
Conv Dispo & Conviction & non-black & 13 & 12.5 & 11.7 & 2.6 \\ 
  Conv Dispo & Conviction & black & 15.5 & 14.4 & 16.3 & 2.7 \\ 
   \hline
Conv Dispo & Booking & non-black & 31.1 & 23.1 & 19 & 3 \\ 
  Conv Dispo & Booking & black & 40.9 & 24.3 & 30.3 & 3.2 \\ 
   \hline
Conv Dispo & Difference & non-black & 18.1 * & 10.6 * & 7.3 * & 0.4 * \\ 
  Conv Dispo & Difference & black & 25.4 * & 9.9 * & 14 * & 0.5 * \\ 
   \hline
\end{tabular}
\caption{Comparison of rate per 100, disaggregated by race-- of receiving a charge-based exclusion, a charge-based bump-up, and average recommendation level for the PSA calculated using different sets of input charges.} 
\label{tab:all-comparison-race}
\end{table}


==> all-comparison.tex <==
% latex table generated in R 3.5.1 by xtable 1.8-4 package
% Wed Dec  4 11:33:45 2019
\begin{table}[ht]
\centering
\begin{tabular}{llllll}
 Subset & Charges & exclusions & bump-ups & nvca & rec \\ 
  \hline
All Cases & Conviction & 8.7 & 9.1 & 9.3 & 2.5 \\ 
  All Cases & Booking & 29.4 & 23.7 & 20.2 & 3 \\ 
  All Cases & Difference & 20.7 * & 14.6 * & 10.8 * & 0.5 * \\ 
   \hline
\hline
Conv Dispo & Conviction & 14.1 & 13.4 & 13.8 & 2.6 \\ 
  Conv Dispo & Booking & 35.5 & 23.7 & 24 & 3.1 \\ 
  Conv Dispo & Difference & 21.3 * & 10.3 * & 10.3 * & 0.4 * \\ 
   \hline
\end{tabular}
\caption{Comparison of rate per 100 of receiving a charge-based exclusion, a charge-based bump-up, and average recommendation level for the PSA calculated using different sets of input charges.} 
\label{tab:all-comparison}
\end{table}


==> comparisons-all-affected.tex <==
% latex table generated in R 3.5.1 by xtable 1.8-4 package
% Mon Aug 19 15:40:15 2019
\begin{table}[ht]
\centering
\begin{tabular}{rrrr}
  \hline
exclusions & bump-ups & nvca & rec \\ 
  \hline
23.00 & 17.60 & 12.00 & 29.50 \\ 
   \hline
\end{tabular}
\caption{Percent of cases for which the PSA component was triggered/higher under the booking charges than under the convictino charges.} 
\label{tab:comparison-all-proportion-affected}
\end{table}


==> comparisons-known-conviction-nogroup.tex <==
% latex table generated in R 3.5.1 by xtable 1.8-4 package
% Wed Dec  4 11:33:45 2019
\begin{table}[ht]
\centering
\begin{tabular}{rlllll}
  \hline
 & Charges & exclusions & bump-ups & nvca & rec \\ 
  \hline
1 & Conviction & 14.1 & 13.4 & 13.8 & 2.6 \\ 
  2 & Booking & 35.5 & 23.7 & 24 & 3.1 \\ 
  3 & Difference & 21.3 * & 10.3 * & 10.3 * & 0.4 * \\ 
   \hline
\end{tabular}
\caption{Comparison of effects of charges on components of PSA for cases for which there are known conviction charges} 
\label{tab:comparison-known-conviction-nogroup}
\end{table}


==> comparisons-known-conviction.tex <==
% latex table generated in R 3.5.1 by xtable 1.8-4 package
% Wed Dec  4 11:33:45 2019
\begin{table}[ht]
\centering
\begin{tabular}{rllllll}
  \hline
 & Charges & group & exclusions & bump-ups & nvca & rec \\ 
  \hline
1 & Conviction & non-black & 13 & 12.5 & 11.7 & 2.6 \\ 
  2 & Conviction & black & 15.5 & 14.4 & 16.3 & 2.7 \\ 
  3 & Booking & non-black & 31.1 & 23.1 & 19 & 3 \\ 
  4 & Booking & black & 40.9 & 24.3 & 30.3 & 3.2 \\ 
  5 & Difference & non-black & 18.1 * & 10.6 * & 7.3 * & 0.4 * \\ 
  6 & Difference & black & 25.4 * & 9.9 * & 14 * & 0.5 * \\ 
   \hline
\end{tabular}
\caption{Comparison of effects of charges on components of PSA by race for cases for which there are known conviction charges} 
\label{tab:comparison-known-conviction-by-race}
\end{table}


==> comparisons-some-conviction-nogroup.tex <==
% latex table generated in R 3.5.1 by xtable 1.8-4 package
% Wed Dec  4 11:33:45 2019
\begin{table}[ht]
\centering
\begin{tabular}{rlllll}
  \hline
 & Charges & exclusions & bump-ups & nvca & rec \\ 
  \hline
1 & Conviction & 11.8 & 11.6 & 11.9 & 2.6 \\ 
  2 & Booking & 32.1 & 22.7 & 22.3 & 3.1 \\ 
  3 & Difference & 20.3 * & 11.1 * & 10.3 * & 0.4 * \\ 
   \hline
\end{tabular}
\caption{Comparison of effects of charges on components of PSA for cases for which some charges resulted in a conviction} 
\label{tab:comparison-conviction-nogroup}
\end{table}


==> comparisons-some-conviction.tex <==
% latex table generated in R 3.5.1 by xtable 1.8-4 package
% Wed Dec  4 11:33:45 2019
\begin{table}[ht]
\centering
\begin{tabular}{rllllll}
  \hline
 & Charges & group & exclusions & bump-ups & nvca & rec \\ 
  \hline
1 & Conviction & non-black & 10.7 & 10.4 & 9.7 & 2.6 \\ 
  2 & Conviction & black & 13.2 & 13.2 & 14.9 & 2.7 \\ 
  3 & Booking & non-black & 27.7 & 21.6 & 17 & 3 \\ 
  4 & Booking & black & 37.8 & 24.2 & 29 & 3.2 \\ 
  5 & Difference & non-black & 17 * & 11.2 * & 7.4 * & 0.4 * \\ 
  6 & Difference & black & 24.6 * & 11 * & 14.1 * & 0.5 * \\ 
   \hline
\end{tabular}
\caption{Comparison of effects of charges on components of PSA by race for cases for which some charges resulted in a conviction} 
\label{tab:comparison-conviction-by-race}
\end{table}


==> court-conv-all-tab.tex <==
% latex table generated in R 3.5.1 by xtable 1.8-4 package
% Thu May  2 15:07:24 2019
\begin{table}[ht]
\centering
\begin{tabular}{|l|r|}
  \hline
  \hline
percent step 2 charges dropped & 24.20 \\ 
  percent step 4 charges dropped & 20.30 \\ 
  percent recommendations 'too high' & 26.60 \\ 
  percent recommended do not release & 21.10 \\ 
   \hline
\end{tabular}
\caption{Percent recommendations changed when using convicted charges} 
\label{tab:court-conv-all}
\end{table}


==> court-conv-tab.tex <==
% latex table generated in R 3.5.1 by xtable 1.8-4 package
% Thu May  2 15:07:24 2019
\begin{table}[ht]
\centering
\begin{tabular}{|l|r|r|}
  \hline
 & non-black & black \\ 
  \hline
percent step 2 charges dropped & 21.80 & 27.30 \\ 
  percent step 4 charges dropped & 19.80 & 20.90 \\ 
  percent recommendations `too high' & 26.50 & 26.70 \\ 
  percent recommended do not release & 19.70 & 22.90 \\ 
   \hline
\end{tabular}
\caption{Percent recommendations changed by race when using convicted charges} 
\label{tab:court-conv}
\end{table}


==> lenient-tab.tex <==
% latex table generated in R 3.5.1 by xtable 1.8-4 package
% Thu May  2 15:07:24 2019
\begin{table}[ht]
\centering
\begin{tabular}{|l|r|r|}
  \hline
 & non-black & black \\ 
  \hline
\% recommendation too high & 29.60 & 34.10 \\ 
  \% unfair do not release & 21.80 & 29.50 \\ 
   \hline
\end{tabular}
\caption{Percent recommendations changed with different DMF} 
\label{tab:lenient}
\end{table}

